How We Refactor and How We Document it? On the Use of Supervised Machine Learning Algorithms to Classify Refactoring Documentation

Refactoring is the art of improving the design of a system without altering its external behavior. Refactoring has become a well established and disciplined software engineering practice that has attracted a significant amount of research presuming that refactoring is primarily motivated by the need to improve system structures. However, recent studies have shown that developers may incorporate refactorings in other development activities that go beyond improving the design. Unfortunately, these studies are limited to developer interviews and a reduced set of projects. To cope with the above-mentioned limitations, we aim to better understand what motivates developers to apply refactoring by mining and classifying a large set of 111,884 commits containing refactorings, extracted from 800 Java projects. We trained a multi-class classifier to categorize these commits into 3 categories, namely, Internal QA, External QA, and Code Smell Resolution, along with the traditional BugFix and Functional categories. This classification challenges the original definition of refactoring, being exclusive to improving the design and fixing code smells. Further, to better understand our classification results, we analyzed commit messages to extract textual patterns that developers regularly use to describe their refactorings. The results show that (1) fixing code smells is not the main driver for developers to refactoring their codebases. Refactoring is solicited for a wide variety of reasons, going beyond its traditional definition; (2) the distribution of refactorings differs between production and test files; (3) developers use several patterns to purposefully target refactoring; (4) the textual patterns, extracted from commit messages, provide better coverage for how developers document their refactorings.

==> Charts/Chart_RQ3_RefactoringOccurrence.tex <==
\begin{figure*}[t]  
\centering 
\begin{tikzpicture}
  \begin{axis}[
    xbar,
    y axis line style = { opacity = 1 },
    axis x line*=bottom,
    axis y line*=left,
    xmin=0, xmax=60,
    tickwidth         = 0pt,
    tick align=inside,
    y=1cm,
    enlarge y limits  = 0.03,
    enlarge x limits  = 0,
    symbolic y coords = { 
    	Rename Class,
        Rename Method,
        Rename Package,
        Extract Interface,
        Push Down Attribute,
        Push Down Method,
        Extract Superclass,
        Pull Up Attribute,
        Pull Up Method,
        Inline Method,
        Move Method,
        Move Attribute,
        Move Class,
        Extract Method,
   	},
   ylabel={Refactoring Operation},
   xlabel={Refactoring Percentage (\%)},
   legend image code/.code={%
   \draw[#1, draw=none,/tikz/.cd,yshift=-0.25em]
        (0cm,1pt) rectangle (6pt,7pt);},
   legend style={
    	at={(0.2,-0.1)},
        anchor=north,
        legend columns=-1,
        /tikz/every even column/.append style={column sep=0.5cm}
        },
    nodes near coords
  ]
   \addplot[fill=gray!25] coordinates {
   		(14.40,Extract Method)
        (13.08,Move Class)
        (4.25,Move Attribute)   
        (2.69,Move Method)
        (2.78,Inline Method) 
        (5.68,Pull Up Method)
        (3.09,Pull Up Attribute)
        (0.88,Extract Superclass)
        (0.48,Push Down Method)
        (0.13,Push Down Attribute)
        (0.54,Extract Interface)
        (1.39,Rename Package)
        (35.47,Rename Method)
        (17.84,Rename Class)
   }; 
  \addplot[fill=black!75] coordinates {
  		(12.97,Extract Method)
        (15.81,Move Class)
        (2.81,Move Attribute)   
        (2.70,Move Method)
        (2.00,Inline Method) 
        (5.94,Pull Up Method)
        (2.27,Pull Up Attribute)
        (0.76,Extract Superclass)
        (0.61,Push Down Method)
        (0.16,Push Down Attribute)
        (0.51,Extract Interface)
        (1.31,Rename Package)
        (42.94,Rename Method)
        (9.19,Rename Class)
   }; 
  
  \legend{After Release, Before Release}
  \end{axis}
\end{tikzpicture}
\caption{Frequency of pre-reslease and post-release refactorings per type} 
\label{Chart:RefactoringsOccurrence}
 \end{figure*} 

==> Charts/Chart_RQ5_RefactoringDistributionPerCategory.tex <==
% TOSEM for V1 
\begin{comment}
\begin{figure*}[p]  
\centering 
\begin{tikzpicture}
  \begin{axis}[
    xbar=0pt,
    %legend pos=outer north east,
    width=9cm,
    height=8cm,
    y axis line style = { opacity = 1 },
    axis x line*=bottom,
    axis y line*=left,
    xmin=0, xmax=35,
    tickwidth         = 0 pt,
    tick align=inside,
    y=6cm,
    enlarge y limits  = auto,
    enlarge x limits  = 0,
    symbolic y coords = { 
         BUGFIX,
         DESIGN,
         FEATURE,
         NON-FUNCTIONAL,
   	},
   ytick=data,
   %grid=major,
   %ymajorgrids=false,
   ylabel={Category},
   xlabel={Refactoring Percentage (\%)},
   legend image code/.code={%
   \draw[#1,draw=none,/tikz/.cd,yshift=-0.25em]
        (0cm,1pt) rectangle (6pt,7pt);},
   % color map from colorbrewer
   %cycle list/Paired,
   % the above only sets the color, need to specify that bars should be filled
%every axis plot/.append style={fill},
   legend style={
    	at={(0.5,-0.05)},
        anchor=north,
        legend columns=5,
        /tikz/every even column/.append style={column sep=0.08cm}
        },
    nodes near coords,
  ]
   % Rename Method
   \addplot[fill=blue] coordinates {
        (32.74,BUGFIX)
        (18.38,DESIGN)
        (27.55,FEATURE)
        (24.57,NON-FUNCTIONAL)
   }; 
   % Extract Method
   \addplot[fill=cyan] coordinates {
        (24.80,BUGFIX)
        (8.47,DESIGN)
        (20.03,FEATURE)
        (17.05,NON-FUNCTIONAL)
   }; 
   % Move Class
   \addplot[fill=violet] coordinates {
        (8.84,BUGFIX)
        (24.84,DESIGN)
        (13.64,FEATURE)
        (16.11,NON-FUNCTIONAL)
   };
   % Rename Class
   \addplot[fill=magenta] coordinates {
        (10.87,BUGFIX)
        (9.81,DESIGN)
        (12.31,FEATURE)
        (13.02,NON-FUNCTIONAL)
   };
    % Pull Up Method
   \addplot[fill=purple] coordinates {
        (5.63,BUGFIX)
        (6.80,DESIGN)
        (6.75,FEATURE)
        (7.87,NON-FUNCTIONAL)
   };
      % Move Attribute
   \addplot[fill=pink] coordinates {
        (4.23,BUGFIX)
        (7.27,DESIGN)
        (4.26,FEATURE)
        (5.30,NON-FUNCTIONAL)
   };
      % Move Method
   \addplot[fill=orange] coordinates {
        (3.74,BUGFIX)
        (12.03,DESIGN)
        (4.68,FEATURE)
        (2.92,NON-FUNCTIONAL)
   };
      % Inline Method
   \addplot[fill=yellow] coordinates {
        (3.61,BUGFIX)
        (3.12,DESIGN)
        (3.04,FEATURE)
        (3.77,NON-FUNCTIONAL)
   };
       % Pull Up Attribute
   \addplot[fill=olive] coordinates {
        (2.53,BUGFIX)
        (3.02,DESIGN)
        (3.37,FEATURE)
        (4.31,NON-FUNCTIONAL)
   };
       % Remaining
   \addplot[fill=green!50] coordinates {
        (3.01,BUGFIX)
        (6.27,DESIGN)
        (4.36,FEATURE)
        (5.07,NON-FUNCTIONAL)
   };
   
  \legend{Rename Method, Extract Method, Move Class, Rename Class, Pull Up Method, Move Attribute, Move Method, Inline Method, Pull Up Attribute, Remaining}
  \end{axis}
\end{tikzpicture}
\caption{Distribution of refactoring types per category} 
\label{fig:ref_dist_class}
 \end{figure*} 
 
 \end{comment}
 
 % TOSEM for V2 
 \begin{comment}
\begin{figure*}[t]  
\centering 
\begin{tikzpicture}
\begin{axis}[
    ybar stacked,
    height=11cm,
    width=18cm,
    percentage plot,
    bar width=0.55cm, % increased from 0.3cm
    xticklabels from table={\dataA}{Category}, % read ticklabels from first column
    xtick=data,
    x tick label style={
      rotate=45,
      anchor=east, 
      xshift=-1.5mm, yshift=-2mm
    },
    legend style={
      at={(0.5,-0.44)},
      anchor=south,
      legend columns=-1
      },
]

    \addplot [fill=cyan]  table[percentage series=1] {\dataA};
    \addplot [fill=pink]                 table[percentage series=2] {\dataA};
    \addplot [fill=storeClusterComponent]       table[percentage series=3] {\dataA};
    \addplot [fill=dbscan]       table[percentage series=4] {\dataA};
    \addplot [fill=constructCluster]       table[percentage series=5] {\dataA};

 

    % plot just to add total
    \addplot [forget plot,nodes near coords align=above] table[x expr=\coordindex,y expr=0.0001,meta=sum]{\dataA};

    \legend{\strut Functional, \strut BugFix, External QA, Internal QA, Code Smell Resolution}
\end{axis}
\end{tikzpicture}
\caption{Distribution of refactoring types per category} 
\label{fig:ref_dist_class}
\end{figure*}
\end{comment}
 
\begin{comment}
%%%%%%%%%5

\begin{figure*}[h]  
\centering 
\begin{tikzpicture}
\begin{axis}[
    ybar stacked,
    height=11cm,
    width=18cm,
    percentage plot,
    bar width=0.55cm, % increased from 0.3cm
    xticklabels from table={\dataB}{File}, % read ticklabels from first column
    xtick=data,
    x tick label style={
      rotate=45,
      anchor=east, 
      xshift=-1.5mm, yshift=-2mm
    },
    legend style={
      at={(0.5,-0.44)},
      anchor=south,
      legend columns=-1
      },
]

    \addplot [fill=pink] table[percentage series=1] {\dataB};
    \addplot [fill=constructCluster] table[percentage series=2] {\dataB};
   

    % plot just to add total
    %\addplot [forget plot,nodes near coords align=above] table[x expr=\coordindex,y expr=0.0001,meta=sum]{\dataB};

    \legend{\strut Production File, \strut Test File}
\end{axis}
\end{tikzpicture}
\caption{Distribution of refactoring types per source file types} 
\label{fig:ref_prod_test}
\end{figure*}
\end{comment}




% TOSEM for V2
\begin{comment}


\begin{figure*}[p]  
\centering 
\begin{tikzpicture}
\begin{scope}[scale=0.65]
  \begin{axis}[
    xbar=0pt,
    %legend pos=outer north east,
    width=12cm,
    height=6cm,
    y axis line style = { opacity = 1 },
    axis x line*=bottom,
    axis y line*=left,
    xmin=0, xmax=30,
    tickwidth         = 0 pt,
    tick align=inside,
    y=1cm,
    enlarge y limits  = auto,
    enlarge x limits  = 0,
    symbolic y coords = { 
         Rename Attribute,
         Rename Variable,
         Rename Method,
         Extract Method,
         Move Attribute,
         Rename Parameter,
         Move Class,
         Move Method, 
         Pull Up Method,
         Extract Variable, 
         Rename Class,
         Extract \& Move Method,
         Pull Up Attribute,
         Push Down Method,
         Inline Method,
         Extract Class,
         Move \% Rename Class,
         Extract Superclass,
         Inline Variable,
         Push Down Attribute,
         Move Source Folder, 
         Parameterize Variable,
         Replace Variable w/ Attribute,
         Change Package,
         Extract Interface,
         Extract Subclass,
         Move \& Rename Attribute,
         Replace Attribute,
   	},
   ytick=data,
   %grid=major,
   %ymajorgrids=false,
   ylabel={Category},
   xlabel={Refactoring Percentage (\%)},
   legend image code/.code={%
   \draw[#1,draw=none,/tikz/.cd,yshift=-0.25em]
        (0cm,1pt) rectangle (6pt,7pt);},
   % color map from colorbrewer
   %cycle list/Paired,
   % the above only sets the color, need to specify that bars should be filled
%every axis plot/.append style={fill},
   legend style={
    	at={(0.3,-0.05)},
        anchor=north,
        legend columns=5,
        /tikz/every even column/.append style={column sep=0.08cm}
        },
    nodes near coords,
  ]
   %  Production
   \addplot[fill=pink] coordinates {
         (20.76,Rename Attribute)
         (12.11,Rename Variable)
         (10.78,Rename Method)
         (7.54,Extract Method)
         (7.53,Move Attribute)
         (6.57,Rename Parameter)
         (6.25,Move Class)
         (5.15,Move Method)
         (3.77,Pull Up Method)
         (3.46,Extract Variable)
         (2.87,Rename Class)
         (2.01,Extract \& Move Method)
         (1.93,Pull Up Attribute)
         (1.58,Push Down Method)
         (1.18,Inline Method)
         (0.96,Extract Class)
         (0.85,Move \% Rename Class)
         (0.75,Extract Superclass)
         (0.69,Inline Variable)
         (0.67,Push Down Attribute)
         (0.62,Move Source Folder) 
         (0.58,Parameterize Variable)
         (0.47,Replace Variable w/ Attribute)
         (0.30,Change Package)
         (0.29,Extract Interface)
         (0.15,Extract Subclass)
         (0.03,Move \& Rename Attribute)
         (0.018,Replace Attribute)
        
   };
   % Test
   \addplot[fill=constructCluster] coordinates {
         (2.77,Rename Attribute)
         (16.65,Rename Variable)
         (29.16,Rename Method)
         (11.76,Extract Method)
         (2.19,Move Attribute)
         (1.02,Rename Parameter)
         (2.26,Move Class)
         (10.18,Move Method)
         (5.24,Pull Up Method)
         (3.77,Extract Variable)
         (1.33,Rename Class)
         (3.33,Extract \& Move Method)
         (3.11,Pull Up Attribute)
         (0.14,Push Down Method)
         (1.19,Inline Method)
         (1.41,Extract Class)
         (0.45,Move \% Rename Class)
         (0.64,Extract Superclass)
         (0.59,Inline Variable)
         (0.03,Push Down Attribute)
         (0,Move Source Folder) 
         (1.02,Parameterize Variable)
         (1.55,Replace Variable w/ Attribute)
         (0,Change Package)
         (0.02,Extract Interface)
         (0.02,Extract Subclass)
         (0.05,Move \& Rename Attribute)
         (0.05,Replace Attribute)
   }; 
  
   
  \legend{Production file, Test file}
  \end{axis}
  \end{scope}
\end{tikzpicture}
\caption{Distribution of refactoring types per category} 
\label{fig:ref_dist_class}
 \end{figure*} 
 
\end{comment}

==> Tables/Table_CommitsClassification.tex <==
\begin{table*}
  \centering
	 \caption{Characteristics of commit classification studies}
	 \label{Table:Commits Classification}
\begin{sideways}
%\begin{adjustbox}{width=1.2\textwidth,center}
\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lcccclll}\hline
\toprule
\bfseries Study & \bfseries Year & \bfseries Single/Multi-labeled & \bfseries Manual/Automatic & \bfseries Classification Method & \bfseries Category & \bfseries Training Size & \bfseries Result \\
\midrule
\citeo{article} & 2006 & Yes/No & No/Yes  & Machine Learning Classifier & Swanson's category & 400 commits (1 participant) & Accuracy: 70\% \\ & & & & & Administrative &  \\  \hline 
 \citep{4686322} & 2008 & Yes/No & No/Yes & Keywords-based Search & Forward Engineering & 1088 commits &  F-Measure: 76\% \\ & & & & & Reengineering \\ & & & & & Corrective Engineering \\ & & & & & Management &  \\ \hline
\citep{Hassan:2008:ACC:1363686.1363876} & 2008 & Yes/No  & No/Yes & Automated Classifier & Bug Fixing & 18 commits (6 participants) & Agreement: 70\%  \\ & & & & & General Maintenance  \\ & & & & & Feature Introduction &  \\
\hline
\citep{Hindle:2008:LCT:1370750.1370773} & 2008 & Yes/Yes & Yes/No & Systematic Labeling & Swanson's category & 2000 commits & Not mentioned \\ & & & & & Feature Addition \\ & & & & & Non-Functional &  \\ \hline 
 \citep{5090025} & 2009 & Yes/No & No/Yes & Machine Learning Classifier & Swanson's category & 2000 commits & F-Measure: 50\%  \\ & & & & & Feature Addition \\ & & & & & Non-Functional &   \\ \hline
 \citep{Hindle:2011:ATN:1985441.1985466} & 2011 & Yes/Yes & No/Yes & Machine Learning Classifier  & Non-Functional & Not Mentioned & Receiver Operating  \\ & & & & & %Mulan's Multi-label Classifier 
&  & Characteristic up to 80\% 
\\ & & & & & &  \\ \hline
\citep{Mauczka2012} & 2012 & Yes/No & No/Yes  & Subcat tool & Swanson's category & 21 commits (5 participants) & Precision: 92\%  \\ & & & & & Blacklist & &  Recall: 85\%  \\ & & & & & &   \\ \hline
 \citep{Tsantalis:2013:MES:2555523.2555539} & 2013 & Yes/No & Yes/No & Systematic Labeling & Code Smell Resolution & Not Mentioned & Manual \\ & & & & & Extension \\ & & & & & Backward Compatibility \\ & & & & & Abstraction Level Refinement &  \\ \hline
\citep{7180125} & 2015 & Yes/Yes & Yes/No & Systematic Labeling & Swanson's category & 967 commits & Manual \\ & & & & & \citep{4686322} category \\ & & & & & Non-Functional &  \\ \hline
 \citep{YAN2016296} & 2016 & Yes/Yes  & No/Yes &  Topic Modeling & Swanson's category & 80 commits (5 participants) & F-Measure: 0.76\% \\ \hline
 \citep{Chavez:2017:RAI:3131151.3131171} & 2017 & Yes/No & Yes/No & Systematic Labeling & Floss Refactoring & sample of 2119 & Manual \\ & & & & & Root-canal Refactoring & \\ \hline
 \citep{cedrim2017understanding} & 2017 & Yes/No & Yes/No & Systematic Labeling & Floss Refactoring & part of sample of 2584 & Manual \\ & & & & & Root-canal Refactoring & \\ \hline
 \citep{Levin:2017:BAC:3127005.3127016} & 2017 & Yes/No & No/Yes & Machine Learning Classifier & Swanson's category & 1151 Commits & Accuracy: 73\% \\
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{sideways}
\end{table*}


==> Tables/Table_CommitsMessageExample.tex <==
% NEW FORMAT
\begin{table*}
  \centering
	 \caption{Commits message examples classified by category}
	 \label{Table:Commits_Messages_Example}
\begin{sideways}
%\begin{adjustbox}{width=1.2\textwidth,center}
\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{llll}\hline
\toprule
\bfseries Category & \bfseries Subcategory & \bfseries Refactoring Operation & \bfseries Commit Messages \\
\midrule
\\
Functional & Feature Addition & Rename \& Extract Method & Implementation of the feature to allow user to add custome exception. Code refactoring for various modules. Incorporated Fabios old review comment. \\ \\ & Feature Modification & Rename Method &  Feature \#5157 - refactoring of album view page (adding some string templates) (modifying homepage) (modifying the view of a photo) \\ & & & (fixing search result display problems) \\ \\ & Feature Deletion &  Pull Up Attribute & Refactored the sauce test class to a base and subclass with test content. Reused sauce base test class to run session id and job-name printing test \\ & & & and checking output by capturing stdout. The nature of the feature being tested forced some unorthodox testing. Also removed build id update from \\ & & & the SauceOnDemandTestListener class to give user the freedom to set their own. In the earlier setup the Jenkins tag was   overwriting the user set one \\ & & & causing odd behaviour.\\ \\ \hline \\

BugFix & Bug Resolution & Extract Method & Refactoring of SlidingWindow class in RR to reduce complexity and  fix important bug \\ \\ & Bug Resolution & Rename Method & Fixed a bug in Extract Function refactoring. \\ \\ & Bug Resolution & Extract Method & Refactor the code to fix bug 256238,Shouldn't update figure before inserting extended item such as Chart in library editor. \\ \\ & Debugging & Move \& Rename Class & Renaming and refactoring towards debugging  functionality. \\ \\ & Bug Localization & Move Method & Moved generateObjects() from AbstractFunction to FunctionHelper. More natural. Updated Wiki docs to reflect this. Found a bug   with \\ & & & using variables in predicates. commented out the test case that breaks. Added some test cases that are more complicated uses of ScriptEngine.\\ \\ \hline \\

Code Smell  &  Long Method & Extract Method & MongoStore: Refactor to avoid long methods \\ \\ & Duplicate Code & Extract Method & Minor refactoring to remove duplicate code \\ \\ & Data Class & Move Class & Refactoring of core data classes. Implementation of RefactoringRegistry.\\ \\ & Feature Envy & Move Method & Introduced adjuncts from stapler - fixed the feature envy problem in the version computation. \\ \\ \hline \\

Internal & Inheritance & Move Attribute, Rename \& Inline Method & Refactoring of filters to make better use of  inheritance hierarchy.\\ \\ & Polymorphism & Move Attribute, Rename \& Inline Method & Refactored to remove Classifier factory pattern and allow for model polymorphism.\\ \\ & Coupling Improvement & Extract Interface & Removes tight coupling between managed service and heartbeat notification. \\ \\ & Cohesion Improvement & Extract Method & Addresses issue \#11 where a general refactor is needed to improve the cohesion of the creation of property value mergers.\\ \\  \hline \\

External & Testability & Extract Method & Minor refactoring for better testability without the need to generate intermediary files. \\ \\ & Usability & Rename Method & Refactor: Remove redundant method names, improve usability. \\ \\ & Performance & Extract Method & 
Improve performance of MessageSource condition.\\ \\ & Reusability & Move Method & Refactored for better reusability. \\ \\ & Readability & Extract Method & Refactoring mostly for readability (and small performance improvement). \\
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{sideways}
\end{table*}








% OLD FORMAT
\begin{comment}
\begin{table*}
  \centering
	 \caption{Commits Message Example}
	 \label{Table:Commits_Messages_Example2}
\begin{sideways}
%\begin{adjustbox}{width=1.0\textwidth,center}
\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lcccc}
\toprule
\bfseries Category & \bfseries Subcategory & \bfseries \begin{tabular}[c]{@{}l@{}}Refactoring Operation\end{tabular}                                                                                                                                                           & \bfseries \begin{tabular}[c]{@{}l@{}}Commit Messages\end{tabular}                                                                                                                                                               \\ 
\midrule
Feature  & \begin{tabular}[c]{@{}l@{}}Feature Addition\\    \\    \\   Feature Modification\\    \\    \\    Feature Deletion\end{tabular}                                                                                        & \begin{tabular}[c]{@{}l@{}}Rename \& Extract Method\\    \\    \\   Rename Method\\    \\    \\    Pull Up Attribute\end{tabular}                                                                              & \begin{tabular}[c]{@{}l@{}}\\ Implementation of the feature to allow user to add custome exception. Code refactoring for various modules. Incorporated Fabios’s old\\   review comment. \\    \\   Feature \#5157 - refactoring of album view page (adding some string templates) (modifying homepage) (modifying the view of a photo)\\   (fixing search result display problems)\\    \\   Refactored the sauce test class to a base and subclass with test content. Reused sauce base test class to run session id and job-name printing test and checking output by capturing stdout. \\ The nature of the feature being tested forced some unorthodox testing. Also removed build id update from the SauceOnDemandTestListener class to give user the freedom to set their own.\\ In the earlier setup the Jenkins tag was   overwriting the user set one causing odd behaviour.\\ \end{tabular} \\ \\ \hline

BugFix   & \begin{tabular}[c]{@{}l@{}}Bug Resolution \\    \\   Bug   Resolution \\    \\   Bug Resolution \\    \\       Debugging\\    \\   Bug Localization\end{tabular}                                                    & \begin{tabular}[c]{@{}l@{}}Extract Method\\    \\   Rename Method\\    \\   Extract Method \\    \\       Move \& Rename Class\\    \\   Move Method\end{tabular}                                       & \begin{tabular}[c]{@{}l@{}}\\ Refactoring of SlidingWindow class in RR to reduce complexity and  fix important bug, \\    \\   Fixed a bug in Extract Function refactoring.\\    \\   Refactor the code to fix bug 256238,Shouldn't update figure before inserting extended item such as Chart in library editor\\    \\   Renaming and refactoring towards debugging  functionality\\    \\   Moved generateObjects() from AbstractFunction to FunctionHelper. More natural. Updated Wiki docs to reflect this. Found a bug   with using variables in predicates. \\ commented out the test case that breaks. Added some test cases that are more complicated uses of ScriptEngine.
\end{tabular}                                               \\ \\ \hline
Design   & \begin{tabular}[c]{@{}l@{}}\\ Code Smell Resolution\\    \\   Code Smell Resolution\\    \\   Code Smell Resolution\\    \\ Code Smell Resolution \\   \\ Inheritance \\    \\        Polymorphism\end{tabular} & \begin{tabular}[c]{@{}l@{}}\\Extract Method\\    \\   Extract Method\\    \\   Move Class\\    \\ Move Method \\ \\   Move Attribute, Rename \& Move Method\\    \\   Move Attribute, Rename \& Inline Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}\\ MongoStore: Refactor to avoid long methods\\    \\   Minor refactoring to remove duplicate code\\    \\   Refactoring of core data classes. Implementation of RefactoringRegistry.\\    \\ Introduced adjuncts from stapler - fixed the feature envy problem in the version computation. \\ \\   Refactoring of filters to make better use of  inheritance hierarchy.\\    \\       Refactored to remove Classifier factory pattern and allow for model polymorphism.
\end{tabular}  
\\ \\  \hline

Non-Functional & \begin{tabular}[c]{@{}l@{}}\\Testability\\    \\   Usability\\    \\   Performance\\    \\   Reusability \\    \\   Readability\end{tabular}                                                                                          & \begin{tabular}[c]{@{}l@{}}\\ Extract Method \\    \\   Rename Method\\    \\   Extract   Method \\    \\   Move Method \\    \\   Extract Method\end{tabular}                                                       & \begin{tabular}[c]{@{}l@{}}\\ Minor refactoring for better testability without the need to generate intermediary files.\\    \\   Refactor: Remove redundant method names, improve usability. \\   \\     Improve performance of MessageSource condition.\\   \\   Refactored for better reusability.\\    \\   Refactoring mostly for readability (and small performance improvement)\end{tabular}   \\ \\               
\bottomrule
\end{tabular}
\end{adjustbox}
\end{sideways}
\end{table*}

\end{comment}

==> Tables/Table_RefactoringDetectionTools.tex <==
\begin{table*}%[h!]
\begin{center}
\caption{Characteristics of refactoring detection studies}
\label{Table:RelatedWorkTools}
%\begin{sideways}
\begin{adjustbox}{width=1.0\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lllll}\hline
\toprule
\bfseries Study & \bfseries Year & \bfseries Refactoring Tool & \bfseries Detection Technique & \bfseries No. of Refactoring \\
\midrule
Dig et al. \citep{Dig2006} & 2006 & Refactoring Crawler & Syntactic \& Semantic analysis &  7  \\
Weissgerber \& Diehl \citep{4019578} & 2006 & Signature-Based Refactoring Detector & Signature-based analysis & 10 \\
Zhenchang \& Eleni \citep{Xing:2008:JTS:1370175.1370203} & 2008 & JDevAn & Design Evolution analysis &  Not Mentioned  \\
Hayashi et al. \citep{hayashi2010search} & 2010 & Search-Based Refactoring Detector & Graph-based heuristic search & 9 \\
Kim et al. \citep{5609577,Kim:2010:RRR:1882291.1882353} & 2010 & Ref-Finder & Template-based rules reconstruction technique & 63 \\
Silva \& Valente \citep{7962377} & 2017 & RefDiff & Static analysis \& code similarity & 13 \\
Tsantalis et al. \citep{tsantalis2018accurate} & 2018  & RefactoringMiner & Design Evolution analysis & 28 \\
\bottomrule
\end{tabular}
\end{adjustbox}
%\end{sideways}
\end{center}
\end{table*}

==> Tables/Table_RefactoringTypes.tex <==
\begin{table*}[t]
\begin{center}
\caption{Refactoring Types (Extracted from  \cite{Fowler:1999:RID:311424}) }
\label{Table:refactoring_types}
%\begin{adjustbox}
\begin{adjustbox}{width=1.0\textwidth,center}
 \begin{tabular}{ lll } \hline
 %\begin{tabular}{l L{130mm}}
  \toprule
  \bfseries Refactoring Type &  \bfseries Description  \\
  \midrule
    (1) Change Package & Change package involves several package-level operations (Move, Rename, Split, Merge).\\
    (2) Extract \& Move Method &  Turn the code fragment into a method whose name explains the purpose of the method and move it to class on which it is defined.\\
    (3) Extract Class &  A class does a work of two classes. Create a new class and move relevant fields and methods to the new class. \\
    (4) Extract Interface &  Several clients use the same subset of a class's interface, or two classes have part of their interfaces in common. 
Extract the subset into an interface.\\ 
    (5) Extract Method &  A code fragment that can be grouped together.
Turn the fragment into a method whose name explains the purpose of the method.    \\
    (6) Extract Subclass & A class has features used only in some instances. Create subclass for that subset of features. \\
    (7) Extract Superclass & There are two classes with similar features. Create a superclass and move the common features to the superclass. \\
    (8) Extract Variable & Turn the fragment into a method whose name explains the purpose of the method. \\
    (9) Inline Method & When method's body is just as clear as its name.
Put the method's body into the body of its callers and remove the method. \\ 
    (10) Inline Variable & When a variable is just as clear as its name. Put the variable into the body of its callers and remove the variable. \\
     (11) Move \& Rename Attribute & Move attribute into another class and change the name of the attribute. \\
    (12) Move \& Rename Class &  Move all class features into another class and change the name of the class.\\
    (13) Move Attribute &  A field is, or will be, used by another class more than the class on which it is defined.\\
    (14) Move Class &  A class isn't doing very much. Move all its features into another class and delete it. \\
    (15) Move Method &  A method is, or will be, using or used by more features of another class than the class on which it
is defined.  \\
    (16) Move Source Folder &  Move a source folder to a different folder. \\
    %(4) Rename Package & High & The name of a package does not reveal its purpose. Change the name of the package.  \\ 
    (17) Parameterize Variable &  When a variable is changed to be a parameter of a method. \\
     (18) Pull Up Attribute &   Two subclasses have the same field. Move the field to the superclass. \\ 
     (19) Pull Up Method &   If at least two subclasses share an identical method, move it to the superclass.\\ 
     (20) Push Down Attribute &   A field is used only by some subclasses. Move the field to those subclasses. \\
     (21) Push Down Method &  The Behavior on a superclass is relevant only for some of its subclasses. Move it to those subclasses.  \\ 
     (22) Rename Attribute &  The name of an attribute does not reveal its purpose. Change the name of the attribute.\\
    (23) Rename Class &  The name of a class does not reveal its purpose. Change the name of the class. \\
    (24) Rename Method & The name of a method does not reveal its purpose. Change the name of the method. \\
    (25) Rename Parameter &  The name of a parameter does not reveal its purpose. Change the name of the parameter.\\
    (26) Rename Variable & The name of a variable does not reveal its purpose. Change the name of the variable. \\
    (27) Replace Attribute &  An attribute is replaced with another attribute. \\
    (28) Replace Variable with Attribute &  A variable is replaced with an attribute.\\
  \bottomrule
  \end{tabular}
  \end{adjustbox}
  \end{center}
\end{table*}

==> Tables/Table_SummaryEmpiricalStudy.tex <==

\begin{table*}[!htbp]
\begin{center}
\caption{Summary of the empirical study design.}
\label{Table:Summary of the empirical study design}
\begin{tabular}{llll}
\toprule
%\multirow{2}{*}[-3pt]{\textbf{Research question}}   & \multicolumn{2}{c}{\textbf{Reference}} \\ 
\textbf{Research question}   & \textbf{Reference} \\
        %\cmidrule{2-3} 
     % &   \textbf{Automated} & \textbf{Manual}  \\ 
         \midrule
    RQ1: Motivation behind refactoring  & Figures~\ref{fig:commit_classification}, ~\ref{fig:commit_classification_prodtest}, ~\ref{fig:Example of Design},~\ref{fig:Example of code smell},~\ref{fig:Example of Non-Functional},~\ref{fig:Example of Feature},~\ref{fig:Example of BugFix}, Tablse~\ref{Table:Commits_Messages_Example},~\ref{Table:prod_vs_test_v2}  \\
    RQ2: Refactoring documentation  & Tables~\ref{Table:GeneralPatterns}, ~\ref{Table:SpecificPatterns_1},~\ref{Table:TopGenericKeywords},~\ref{Table:TopSpecificKeywords}, Figures~\ref{Figure:violin-plots-refacoring-occurrences},~\ref{fig:wordcloud},~\ref{fig:Refactoring Operation}  \\ 
    %RQ3: Refactoring operations perform on production and test code  & Table ~\ref{Table:prod_vs_test_v2}  \\ 

    %RQ3: Refactoring contributors & Fig~\ref{fig:Top_Rest_Ref_NonRefCommits_Uncombined}%~\ref{fig:Top_Rest_Ref_NonRef_Commits_Combined} 
    %& Fig~\ref{fig:Refactoring_Contributors}  \\ 
    %RQ4: Correlation between refactoring and project releases & Fig~\ref{fig:Refactoring_Density_Release_Point_Comparison.},~\ref{fig:Refactoring_Operation_Production},~\ref{fig:Refactoring_Operation_Test},~\ref{Chart:RefactoringsOccurrence}, Table~\ref{Table:Release_Point_Comparision}   & Fig~\ref{fig:Refactoring_Activity_Comparison_Hadoop },~\ref{fig:Refactoring_Activity_Comparison_OrientDB },~\ref{fig:Refactoring_Activity_Comparison_Camel } \\ 
    %RQ5: Correlation between refactoring and test hoptspots  & Fig ~\ref{fig:Refactoring_Density_Test_Point_Comparison.},~\ref{fig:Refactoring_Operation_Production_Test_Comparision},~\ref{fig:Refactoring_Operation_Test_Test_Comparision} & Fig~\ref{fig:Refactoring_Activity_Comparison_Test_Hadoop },~\ref{fig:Refactoring_Activity_Comparison_Test_OrientDB },~\ref{fig:Refactoring_Activity_Comparison_Test_Camel } \\
        \bottomrule
\end{tabular} 
\end{center}
\end{table*}
